Learning Regular Languages over Large Ordered Alphabets

This work is concerned with regular languages defined over large alphabets, either infinite or just too large to be expressed enumeratively. We define a generic model where transitions are labeled by elements of a finite partition of the alphabet. We then extend Angluin's L* algorithm for learning regular languages from examples for such automata. We have implemented this algorithm and we demonstrate its behavior where the alphabet is a subset of the natural or real numbers. We sketch the extension of the algorithm to a class of languages over partially ordered alphabets.

==> AngluinsLearning.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%
%%     Learning Angluin's L*
%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%\section{Learning Concrete Automata}

We briefly survey Angluin's $L^*$ algorithm \cite{Angluin87} for learning regular sets from membership queries and counter-examples, with slightly modified definitions to accommodate for its symbolic extension. Let $\S$ be a finite alphabet and let $\S^*$ be the set of sequences (words) over $\S$. Any order relation $<$ over $\S$ can be naturally lifted to a lexicographic order over $\S^*$. \comment{ that we denote by $<_l$.} With a language $L\se \S^*$ we associate a \emph{characteristic function} $f:\S^*\to\{+,-\}$, where $f(w) = +$ if the word $w \in \S^{*}$ belongs to $L$ and $f(w) = -$, otherwise. 

A \emph{deterministic finite automaton}  over $\S$ is a tuple $\A = (\S, Q, \d,
q_0,F)$, where $Q$ is a non-empty finite set of \emph{states}, $q_0 \in Q$ is
the \emph{initial} state, $\d : Q \times \S \to Q$ is the \emph{transition
function}, and $F \se Q$ is the set of \emph{final} or \emph{accepting} states.
The transition function $\d$ can be extended to $\d: Q \times \S^{*} \to Q$,
where $\d(q,\e) = q$, and $\d(q,u \cdot a) = \d(\d(q,u),a)$ for $q \in Q$, $a
\in \S$ and $u \in \S^{*}$. A word $w\in \S^{*}$ is \emph{accepted} by $\A$ if
$\d(q_0,w) \in F$, otherwise $w$ is \emph{rejected}. The language recognized by
$\A$ is the set of all accepted words and is denoted by $L(\A)$. 

% Learner
Learning algorithms, represented by the \emph{learner}, are designed to infer
an unknown regular language $L$ (the \emph{target language}). The learner aims
to construct a finite automaton that recognizes $L$ by gathering
information from the \emph{teacher}. The \emph{teacher} knows $L$ and can
provide information about it. It can answer two types of queries:
\emph{membership queries}, i.e., whether a given word belongs to the target
language, and \emph{equivalence queries}, i.e., whether a conjectured automaton
suggested by the learner is the right one. If this automaton fails to accept $L$
the teacher responds to the equivalence query by a \emph{counter-example}, a
word miss-classified by the conjectured automaton.

In the $L^*$ algorithm, the learner starts by asking membership queries. All information provided is suitably gathered in a table structure, the \emph{observation table}. Then, when the information is sufficient, the learner constructs a \emph{hypothesis automaton} and poses an equivalence query to the teacher. If the answer is positive then the algorithm terminates and returns the conjectured automaton. Otherwise the learner accommodates the information provided by the counter-example into the table, asks additional membership queries until it can suggest a new hypothesis and so on, until termination.


A prefix-closed set $ S \uplus R \subset \S^{*} $ is a \emph{balanced $\S$-tree} if $\forall a \in \S$: 1) For every $s \in S$ $s\cdot a \in S\cup R$, and 2)  For every $r\in R$,  $r \cdot a \not \in S\cup R $. Elements of $R$ are called \emph{boundary elements} or \emph{leaves}.
\footnote{We use $\uplus$ for disjoint union.}

% define observation table
\begin{defi} [Observation Table]
An \emph{observation table} is a tuple $T = ( \S, S, R, E, f )$ such that $\S$
is an alphabet, $S \cup R$ is a balanced $\S$-tree, $E$ is a subset of
$\S^{*}$ and $f : (S \cup  R) \cdot E \to \{-, +\}$ is the classification
function, a restriction of the characteristic function of the target language
$L$.
\end{defi}

\ni The set $(S \cup  R) \cdot E$ is the \emph{sample} associated with the
table, that is, the set of words whose membership is known. The elements of $S$
admit a tree structure isomorphic to a \emph{spanning tree} of the transition
graph rooted in the initial state. Each $s\in S$ corresponds to a state $q$ of
the automaton for which $s$ is an \emph{access sequence}, one of the shortest
words that lead from the initial state to  $q$. The elements of $R$ should tell
us about the back- and cross-edges in the automaton and the elements of $E$ are 
``experiments" that should be sufficient to distinguish between states. This
works by associating with every  $s \in S \cup R$ a specialized classification
function $ f_s : E \to \{ - , + \} $, defined as $ f_s (e) = f( s \cdot e)$,
which characterizes the row of the observation table labeled by $s$. To build an
automaton from a table it should satisfy certain conditions.

\begin{defi}[Closed, Reduced and Consistent Tables]
An observation table $T$ is:
    \begin{itemize}
        \item Closed if for every $r \in R$, there exists an $s \in S$, such that $f_r = f_s$;
        \item Reduced if for every $s,s'\in S~f_s\not=f_{s'}$;
        \item Consistent if for every $s, s' \in S$,  $f_{s} = f_{s'}$ implies 
        $ f_{s\cdot a }  = f_{ s'\cdot a }, \forall a \in \S$.
    \end{itemize}
\end{defi}
%
\ni Note that a reduced table is trivially consistent and that for a closed and
reduced table we can define a function $g:R\to S$ mapping every $r\in R$ to the
unique $s\in S$ such that $f_s=f_r$. From such an observation table $T= ( \S, S,
R, E, f )$ one can construct an automaton $\A_T = (\S, Q, q_0, \d, F)$ where $Q
=S$, $q_0=\e$, $F=\{s \in S:f_s(\e) = +\}$ and $$ \d(s,a) = \left\{
\begin{array}{l l} s \cdot a   &  \mbox{ when } s \cdot a \in S\\    g(s\cdot a)
  & \mbox{ when } s \cdot a  \in R \end{array} \right.$$

\ni The learner attempts to keep the table closed at all times.
The table is not closed when there is some $r \in R $ such that $ f_{r}$ is different from $f_{s}$ for all $s \in S $. To close the table, the learner moves $r$ from $R$ to $S$ and adds the $\S$-successors of $r$, i.e., all words $r\cdot a$ for $a\in\S$, to $R$. The extended table is then filled up by asking membership queries until it becomes closed.


% If a table is closed and consistent we can make a conjecture

Variants of the $L^*$ algorithm differ in the way they treat counter-examples, as described in more detail in \cite{BergR04}. The original algorithm \cite{Angluin87} adds all the \emph{prefixes} of the counter-example to $S$ and thus possibly creating inconsistency that should be fixed. The version proposed in \cite{maler1995learnability} for learning $\omega$-regular languages adds all the \emph{suffixes} of the counter-example to $E$. The advantage of this approach is that the table always remains consistent and reduced with $S$ corresponding exactly to the set of states. A disadvantage is the possible introduction of redundant columns that do not contribute to further discrimination between states. The symbolic algorithm that we develop in this paper is based on an intermediate variant, referred to in \cite{BergR04} as the \emph{reduced observation algorithm}, where some prefixes of the counter-example are added to $S$ and some suffixes are added to $E$.



\input{AngluinsLearningexample}

%\clearpage




==> AngluinsLearningexample.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%
%%     L*  Learning Example 
%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\begin{exa} \label{ex:Lstar}
We illustrate the behavior of the $L^{*}$ algorithm while learning a language
$L$ over $\S = \{1,2,3,4,5\}$. We use the tuple $(w,+)$ to indicate a counter-example $w \in
L$ rejected by the conjectured automaton, and $(w,-)$ for the opposite case.
Initially, the observation table is $T_0 = (\S, S, R, E, f)$ with $S = E =
\{\epsilon\}$ and $R = \S$ and we ask membership queries for all words in $(S
\cup R) \cdot E$ to obtain table $T_0$, shown in Fig.~\ref{fig:Angluintables}.
The table is not closed so we move word $1$ to $S$, add its continuations,
$1\cdot\S$ to $R$ and ask membership queries to obtain table $T_1$ which is
now closed. We construct an hypothesis $\A_1$ (Fig.~\ref{fig:AngluinsHA}) from
this table, and pose an equivalence query for which the teacher returns 
counter-example $(3\cdot1,-)$. We add $3\cdot1$ and its prefix $3$ to set $S$ and
add all their continuations to the boundary of the table resulting table
$T_2$ of Fig.~\ref{fig:Angluintables}. This table is not consistent:
two elements $\epsilon$ and $3$ in $S$ are equivalent but their successors 
$1$ and $3\cdot1$ are not. In order to distinguish the two strings we add to $E$
the suffix $1$ and end up with a closed and consistent table $T_3$. The new
hypothesis for this table is $\A_3$, shown in Fig.~\ref{fig:AngluinsHA}. Once 
more the equivalence query will return a counter-example, $(1\cdot3\cdot3,-)$. We
again add the counter-example and prefixes to the table,  ask membership queries
to fill in the table and solve the inconsistency that appears for $1$ and
$1\cdot3$ by adding suffix 3 to the table. The table corresponds now to the
correct hypothesis $\A_5$, and the algorithm
terminates. \qed
\end{exa}


% Observation tables for Angluin
\begin{figure}
    \centering
    \scalebox{.8}{\input{./Figures/Ex_Lstar/ex_Lstar_tables_red.tex}}
    \smallskip
    \caption{Observation tables for Example~\ref{ex:Lstar}.}
    \label{fig:Angluintables}
\end{figure}

% Table with hypothesis automata for Angluin
\begin{figure}
    \centering
    \scalebox{.9}{
    \begin{tabular}{|@{ \extracolsep{\fill} } c | c | c @{ }|}
        \hline
        $\A_1$ & $\A_3$ & $\A_5$\\
        %\hline
	\begin{tabular}{c}
        \input{./Figures/Ex_Lstar/ex_Lstar_h0}
	\end{tabular}
	    &   
	\begin{tabular}{c}
	\input{./Figures/Ex_Lstar/ex_Lstar_h1} 
	\end{tabular}
	    &   
	\begin{tabular}{c}
	\input{./Figures/Ex_Lstar/ex_Lstar_h2} 
	\end{tabular}\\
        \hline\noalign{\smallskip}
    \end{tabular}}
    \caption{Hypotheses for Example~\ref{ex:Lstar}}
    \label{fig:AngluinsHA}
\end{figure}

%\clearpage
   




==> discussion.tex <==
%\section{Discussion}

We have defined a generic algorithmic scheme for automaton learning, targeting  languages over large alphabets that can be recognized by finite symbolic automata having a modest number of states and transitions. Some ideas similar to ours have been proposed for the particular case of parametric languages  \cite{BergJR06} and recently in a more general setting \cite{alph-refinement,local-alph,bb13sigma} including partial evidential support and alphabet refinement during the learning process.

The genericity of our algorithm is due to a semantic approach (alphabet partitions) but of course, each and every domain will have its own semantic and syntactic specialization in terms of the size and shape of the alphabet partitions. In this work we have implemented an instantiation of this scheme for alphabets such as $(\N, \leq)$ and $(\R,\leq)$. 
When dealing with numbers, the partition into a finite number of intervals (and monotone sets in higher dimensions) is very natural and used in many application domains ranging from quantization of sensor readings to income tax regulations. It will be interesting to compare the expressive power and succinctness of symbolic automata with other approaches for representing numerical time series and to compare our algorithm with other inductive inference techniques for sequences of numbers.

As a first excursion into the domain, we have made quite strong assumptions on the nature of the equivalence oracle, which, already for small alphabets, is a bit too strong and pedagogical to be realistic. We assumed that it provides the shortest counter-example and also that it chooses always the minimal available concrete symbol. We can relax the latter (or both) and even omit this oracle altogether and replace it by random sampling, as already proposed in \cite{Angluin87} for concrete learning.
Over large alphabets, it might be even more appropriate to employ probabilistic convergence criteria a-la \emph{PAC learning} \cite{valiant1984theory} and be content with a correct classification of a large fraction of the words, thus tolerating imprecise tracing of boundaries in the alphabet partitions.
This topic is subject to ongoing work. Another challenging research direction is the adaptation of our framework to languages over Boolean vectors.


